An H-theorem for the Brownian motion on the hyperbolic plane

We prove an $H-$theorem for the Brownian motion on the hyperbolic plane with a drift, as studied by Comtet and Monthus; the entropy used here is not the Boltzmann entropy but the R\'enyi entropy, the parameter of which being related in a simple way to the value of the drift.

==> 0176556.tex <==
%auto-ignore
